Experiences Readying Applications for Exascale

The advent of exascale computing invites an assessment of existing best practices for developing application readiness on the world's largest supercomputers. This work details observations from the last four years in preparing scientific applications to run on the Oak Ridge Leadership Computing Facility's (OLCF) Frontier system. This paper addresses a range of topics in software including programmability, tuning, and portability considerations that are key to moving applications from existing systems to future installations. A set of representative workloads provides case studies for general system and software testing. We evaluate the use of early access systems for development across several generations of hardware. Finally, we discuss how best practices were identified and disseminated to the community through a wide range of activities including user-guides and trainings. We conclude with recommendations for ensuring application readiness on future leadership computing systems.

==> figures/pele/pelec-frontier-weak-scaling.tex <==
\begin{figure}
\centering
\begin{tikzpicture}
\begin{semilogxaxis}[
         title=Pele Weak Scaling on Frontier,
  xlabel={Nodes},
  ylabel={Parallel Efficiency (\%)},
  log basis x={2},
  ymin=40, ymax=110,
  %xmin=0, xmax=8192,
  xtick=data,
  legend pos=south west,
  legend columns=1,
  legend style={font=\tiny},
  width=0.9\linewidth, height=0.6\linewidth,
  every axis plot/.append style={thick},
  %/pgf/number format/.cd,
  %      use comma,
  %      1000 sep={},
]

\addplot[mark=*, mark options={solid}, solid,color=blue] coordinates {
(1, 100.00)
(4, 102.0)
(16, 101.35)
(64, 100.08)
(256, 98.65)
(1024, 94.87)
(4096, 88.09)
};

\addplot[mark=*, mark options={solid}, solid,color=red] coordinates {
(1, 100.00)
(4, 97.38)
(16, 96.71)
(64, 96.21)
(256, 94.86)
(1024, 92.42)
(4096, 84.54)
};

\node[anchor=west] (source) at (axis cs:5, 70){68 billion total cells};
      \node (destination) at (axis cs:4000, 88){};
      \draw[->](source)--(destination);

\node[anchor=west] (source) at (axis cs:50, 45){27 billion total cells};
      \node (destination) at (axis cs:4050, 84){};
      \draw[->](source)--(destination);

\legend{PeleC, PeleLMeX}
\end{semilogxaxis}
\end{tikzpicture}
\caption{Weak scaling of premixed flame case: PeleC with one level of AMR, two million cells per GPU; PeleLMeX with two levels of AMR, 0.9 million cells per GPU.}
\label{fig:frontier-weak-scaling-pmf-dodecane}
\end{figure}


